Botnet Detection using Social Graph Analysis

Signature-based botnet detection methods identify botnets by recognizing Command and Control (C\&C) traffic and can be ineffective for botnets that use new and sophisticate mechanisms for such communications. To address these limitations, we propose a novel botnet detection method that analyzes the social relationships among nodes. The method consists of two stages: (i) anomaly detection in an "interaction" graph among nodes using large deviations results on the degree distribution, and (ii) community detection in a social "correlation" graph whose edges connect nodes with highly correlated communications. The latter stage uses a refined modularity measure and formulates the problem as a non-convex optimization problem for which appropriate relaxation strategies are developed. We apply our method to real-world botnet traffic and compare its performance with other community detection methods. The results show that our approach works effectively and the refined modularity measure improves the detection accuracy.

==> wj_macros.tex <==
\usepackage{mathrsfs}

\global\long\def\ra{\rightarrow}
\global\long\def\Ra{\Rightarrow}
\global\long\def\diag{\text{diag}}
\global\long\def\tsum{{\textstyle \sum}}
\global\long\def\dsum{{\displaystyle \sum}}
\global\long\def\tprod{{\textstyle \prod}}
\global\long\def\argmax{\mathop{\rm arg\, max}}


\global\long\def\mb#1{\mathbf{#1}}
\global\long\def\bsy#1{\boldsymbol{#1}}
\global\long\def\mn#1{\mathnormal{#1}}


\global\long\def\ba{\mathbf{a}}
\global\long\def\bb{\mathbf{b}}
\global\long\def\bc{\mathbf{c}}
\global\long\def\bd{\mathbf{d}}
\global\long\def\f{\mathbf{f}}
\global\long\def\bg{\mathbf{g}}
\global\long\def\bh{\mathbf{h}}
\global\long\def\bi{\mathbf{i}}
\global\long\def\bj{\mathbf{j}}
\global\long\def\bk{\mathbf{k}}
\global\long\def\bl{\mathbf{l}}
\global\long\def\bm{\mathbf{m}}
\global\long\def\bn{\mathbf{n}}
\global\long\def\bo{\mathbf{o}}
\global\long\def\bp{\mathbf{p}}
\global\long\def\bq{\mathbf{q}}
\global\long\def\br{\mathbf{r}}
\global\long\def\bs{\mathbf{s}}
\global\long\def\bt{\mathbf{t}}
\global\long\def\bu{\mathbf{u}}
\global\long\def\bv{\mathbf{v}}
\global\long\def\bw{\mathbf{w}}
\global\long\def\bx{\mathbf{x}}
\global\long\def\by{\mathbf{y}}
\global\long\def\bz{\mathbf{z}}


\global\long\def\bA{\mathbf{A}}
\global\long\def\bB{\mathbf{B}}
\global\long\def\bC{\mathbf{C}}
\global\long\def\bD{\mathbf{D}}
\global\long\def\bE{\mathbf{E}}
\global\long\def\bF{\mathbf{F}}
\global\long\def\bG{\mathbf{G}}
\global\long\def\bH{\mathbf{H}}
\global\long\def\bI{\mathbf{I}}
\global\long\def\bJ{\mathbf{J}}
\global\long\def\bK{\mathbf{K}}
\global\long\def\bL{\mathbf{L}}
\global\long\def\bM{\mathbf{M}}
\global\long\def\bN{\mathbf{N}}
\global\long\def\bO{\mathbf{O}}
\global\long\def\bP{\mathbf{P}}
\global\long\def\bQ{\mathbf{Q}}
\global\long\def\bR{\mathbf{R}}
\global\long\def\bS{\mathbf{S}}
\global\long\def\bT{\mathbf{T}}
\global\long\def\bU{\mathbf{U}}
\global\long\def\bV{\mathbf{V}}
\global\long\def\bW{\mathbf{W}}
\global\long\def\bX{\mathbf{X}}
\global\long\def\bY{\mathbf{Y}}
\global\long\def\bZ{\mathbf{Z}}


\global\long\def\bzero{\mathbf{0}}
\global\long\def\bone{\mathbf{1}}


\global\long\def\calA{\mathcal{A}}
\global\long\def\calB{\mathcal{B}}
\global\long\def\calC{\mathcal{C}}
\global\long\def\calD{\mathcal{D}}
\global\long\def\calE{\mathcal{E}}
\global\long\def\calF{\mathcal{F}}
\global\long\def\calG{\mathcal{G}}
\global\long\def\calH{\mathcal{H}}
\global\long\def\calI{\mathcal{I}}
\global\long\def\calJ{\mathcal{J}}
\global\long\def\calK{\mathcal{K}}
\global\long\def\calL{\mathcal{L}}
\global\long\def\calM{\mathcal{M}}
\global\long\def\calN{\mathcal{N}}
\global\long\def\calO{\mathcal{O}}
\global\long\def\calP{\mathcal{P}}
\global\long\def\calR{\mathcal{R}}
\global\long\def\calS{\mathcal{S}}
\global\long\def\calQ{\mathcal{Q}}
\global\long\def\calU{\mathcal{U}}
\global\long\def\calV{\mathcal{V}}
\global\long\def\calW{\mathcal{W}}
\global\long\def\calX{\mathcal{X}}
\global\long\def\calY{\mathcal{Y}}
\global\long\def\calZ{\mathcal{Z}}


\global\long\def\bcalA{\boldsymbol{\mathcal{A}}}
\global\long\def\bcalB{\boldsymbol{\mathcal{B}}}
\global\long\def\bcalC{\boldsymbol{\mathcal{C}}}
\global\long\def\bcalD{\boldsymbol{\mathcal{D}}}
\global\long\def\bcalE{\boldsymbol{\mathcal{E}}}
\global\long\def\bcalF{\boldsymbol{\mathcal{F}}}
\global\long\def\bcalG{\boldsymbol{\mathcal{G}}}
\global\long\def\bcalH{\boldsymbol{\mathcal{H}}}
\global\long\def\bcalI{\boldsymbol{\mathcal{I}}}
\global\long\def\bcalJ{\boldsymbol{\mathcal{J}}}
\global\long\def\bcalK{\boldsymbol{\mathcal{K}}}
\global\long\def\bcalL{\boldsymbol{\mathcal{L}}}
\global\long\def\bcalM{\boldsymbol{\mathcal{M}}}
\global\long\def\bcalN{\boldsymbol{\mathcal{N}}}
\global\long\def\bcalO{\boldsymbol{\mathcal{O}}}
\global\long\def\bcalP{\boldsymbol{\mathcal{P}}}
\global\long\def\bcalR{\boldsymbol{\mathcal{R}}}
\global\long\def\bcalS{\boldsymbol{\mathcal{S}}}
\global\long\def\bcalQ{\boldsymbol{\mathcal{Q}}}
\global\long\def\bcalU{\boldsymbol{\mathcal{U}}}
\global\long\def\bcalV{\boldsymbol{\mathcal{V}}}
\global\long\def\bcalW{\boldsymbol{\mathcal{W}}}
\global\long\def\bcalX{\boldsymbol{\mathcal{X}}}
\global\long\def\bcalY{\boldsymbol{\mathcal{Y}}}
\global\long\def\bcalZ{\boldsymbol{\mathcal{Z}}}


\global\long\def\scrA{\mathscr{A}}
\global\long\def\scrB{\mathscr{B}}
\global\long\def\scrC{\mathscr{C}}
\global\long\def\scrD{\mathscr{D}}
\global\long\def\scrE{\mathscr{E}}
\global\long\def\scrF{\mathscr{F}}
\global\long\def\scrG{\mathscr{G}}
\global\long\def\scrh{\mathscr{h}}
\global\long\def\scrH{\mathscr{H}}
\global\long\def\scrI{\mathscr{I}}
\global\long\def\scrJ{\mathscr{J}}
\global\long\def\scrK{\mathscr{K}}
\global\long\def\scrL{\mathscr{L}}
\global\long\def\scrM{\mathscr{M}}
\global\long\def\scrN{\mathscr{N}}
\global\long\def\scrO{\mathscr{O}}
\global\long\def\scrP{\mathscr{P}}
\global\long\def\scrQ{\mathscr{Q}}
\global\long\def\scrR{\mathscr{R}}
\global\long\def\scrS{\mathscr{S}}
\global\long\def\scrT{\mathscr{T}}
\global\long\def\scrU{\mathscr{U}}
\global\long\def\scrV{\mathscr{V}}
\global\long\def\scrW{\mathscr{W}}
\global\long\def\scrX{\mathscr{X}}
\global\long\def\scrY{\mathscr{Y}}
\global\long\def\scrZ{\mathscr{Z}}


\global\long\def\balpha{\boldsymbol{\alpha}}
\global\long\def\bgamma{\boldsymbol{\gamma}}
\global\long\def\bdelta{{\boldsymbol{\delta}}}
\global\long\def\bepsilon{\boldsymbol{\epsilon}}
\global\long\def\bzeta{\boldsymbol{\zeta}}
\global\long\def\btheta{\boldsymbol{\theta}}
\global\long\def\bth{\boldsymbol{\theta}}
\global\long\def\bkappa{\boldsymbol{\kappa}}
\global\long\def\blambda{\boldsymbol{\lambda}}
\global\long\def\bmu{\boldsymbol{\mu}}
\global\long\def\bnu{\boldsymbol{\nu}}
\global\long\def\bpi{\boldsymbol{\pi}}
\global\long\def\brho{\boldsymbol{\rho}}
\global\long\def\bsigma{\boldsymbol{\sigma}}
\global\long\def\bSigma{\boldsymbol{\Sigma}}


\global\long\def\bxi{\boldsymbol{\xi}}
\global\long\def\btheta{\boldsymbol{\theta}}
\global\long\def\bth{\boldsymbol{\theta}}
\global\long\def\bphi{\boldsymbol{\phi}}
\global\long\def\bpsi{\boldsymbol{\psi}}
\global\long\def\bomega{\boldsymbol{\omega}}


\global\long\def\bXi{\boldsymbol{\Xi}}
\global\long\def\bTheta{\boldsymbol{\Theta}}
\global\long\def\bPhi{\boldsymbol{\Phi}}
\global\long\def\bPsi{\boldsymbol{\Psi}}
\global\long\def\bOmega{\boldsymbol{\Omega}}


\global\long\def\mb#1{\mathbb{#1}}


\global\long\def\mc#1{\mathcal{#1}}
\global\long\def\diag{\mathrm{diag}}


\global\long\def\Tr{\mathrm{Tr}}


\global\long\def\sgn{\mathrm{sgn}}


\global\long\def\lt{}
\global\long\def\rt{}

